ARtonomous: Introducing Middle School Students to Reinforcement Learning Through Virtual Robotics

Typical educational robotics approaches rely on imperative programming for robot navigation. However, with the increasing presence of AI in everyday life, these approaches miss an opportunity to introduce machine learning (ML) techniques grounded in an authentic and engaging learning context. Furthermore, the needs for costly specialized equipment and ample physical space are barriers that limit access to robotics experiences for all learners. We propose ARtonomous, a relatively low-cost, virtual alternative to physical, programming-only robotics kits. With ARtonomous, students employ reinforcement learning (RL) alongside code to train and customize virtual autonomous robotic vehicles. Through a study evaluating ARtonomous, we found that middle-school students developed an understanding of RL, reported high levels of engagement, and demonstrated curiosity for learning more about ML. This research demonstrates the feasibility of an approach like ARtonomous for 1) eliminating barriers to robotics education and 2) promoting student learning and interest in RL and ML.

==> 03-formative.tex <==
\section{Formative Investigation}
We conducted a formative investigation to understand the needs of students and educators in the robotics space and to explore the potential impacts of machine learning and autonomy on their current practice. 

\subsection{Method}
We interviewed 7 middle school robotics educators (3 female; 4 male) who taught robotics in a diverse range of settings (see Table \ref{tab:educators}). Three of these educators worked in  schools where more than half of the students were on free or reduced lunch programs. We also interviewed 6 middle school students (ages 11--13; 1 female, 5 male) who had extensive experience participating in robotics through in- or after-school programs or as a part of FIRST teams.

Our semi-structured interview protocol included questions about experiences teaching and learning robotics, motivators for doing so, and common challenges or points of frustrations. In addition, we solicited feedback on a series of hypothetical scenarios related to autonomous navigation to understand the potential impact of reinforcement learning on everyday educational robotics. 

These interviews took place during the COVID-19 pandemic and were conducted using a video conferencing system. Sessions ranged from 35 minutes to 67 minutes ($M = 50$). The video conferencing software auto-transcribed the sessions, and we manually corrected these transcriptions for later analysis. In analyzing the data, two researchers collaboratively developed a codebook emergent from the data itself, and then iteratively coded the data while updating this codebook until reaching saturation.

\begin{table}[t]
\begin{tabular}{llll}
\hline
\textbf{} & \textbf{Grade} & \textbf{Setting} & \textbf{Low Income} \\ \hline
\textbf{Educator 1} & 6 & FIRST Robotics Coach & No \\
\textbf{Educator 2} & 4--9 & FIRST Robotics Coach & No \\
\textbf{Educator 3} & 6 & FIRST Robotics Coach & No \\
\textbf{Educator 4} & 7 & Biology Classroom & No \\
\textbf{Educator 5} & 6--8 & STEM Classroom & Yes \\
\textbf{Educator 6} & 6 & 6th Grade Classroom & Yes \\
\textbf{Educator 7} & 7--8 & Technology Classroom & Yes \\ \hline
\end{tabular}
\caption{Grade levels and classroom settings for the seven educators who participated in the formative interviews. Here we define educators as working in low-income settings when they reported that more than half of their students were on free or reduced lunch programs.}
\label{tab:educators}
\end{table}

\subsection{Findings and Design Objectives}
From this formative investigation process, we identified two high-level needs and corresponding design objectives. We  discuss separately the potential impacts of autonomous navigation on middle school robotics.

\subsubsection{Need for Access}
First, we found a pervasive challenge in accessing robotics education deriving from cost barriers and time and space constraints. This finding drives a need for more equitable access to robotics education. 

The materials themselves are expensive, and this upfront cost is compounded by a need for multiple sets for a classroom or additional peripherals on top of a base kit. With five of the seven educators specifically pointing to cost as major a challenge, we see that schools and parents alike are often unable to support their students in robotics education due to this price barrier alone.

\begin{quote}
    “Today I was just in a training... and so that was, like, some cool stuff. It's like, how much is that? Oh, it's 200 dollars. Like, okay, that's not going to probably happen.” --Educator 6
\end{quote}

This material cost ultimately means students share the same resources across classes, which limits what educators can do in a class period because they need time for cleanup, and can lead to frustration on the part of a student, who needs to take apart what they've built so the next student can use those same supplies. 

\begin{quote}
    “If I only have one robot, and that we had to keep taking apart every class period so the next class can use it—or even six of them—that becomes a problem.” --Educator 5
\end{quote}

Robotics is similarly constrained by physical space and time. Competition robotics requires a large (8 ft x 4 ft), semi-permanent platform or table that participants build on over the course of the year, and classroom robotics needs an open space free of desks for children to test robots. When students can meet, their time is limited; individual meetings are short, setup and cleanup can occupy a large portion of that time, and there may not be enough meetings over the span of a course to get through all the material. Child 4 is a peer mentor and described how students in his course do not learn programming because there is not enough time to cover both that and hardware. Instead, the instructors provide the students with working code for the robots they build.

\begin{quote}
    “The bad thing is that we only have a year and we only meet once a week…So if it was a full course maybe we'd teach them how to write code. And that's why we write…code and give it to them.” --Child 4
\end{quote}

Ultimately, educators and learners have to pick and choose what content to cover within these time constraints, which leads some educators to choose between emphasizing computing or mechanical engineering. In some cases, they provide students with working code so they can focus on hardware, while others reported working from completed robots, rather than kits, to focus on software.

% We see further issues of access on the side of the educators. Of  the seven educators we interviewed, two had no teaching experience prior to teaching robotics, two had no coding experience, and six had no robotics experience. That is, volunteer robotics coaches are often new to teaching and classroom educators are often new to coding and robotics. Therefore, these coaches often struggled to get support in managing a team, as they do not know how to find administrative information about their program or how to prioritize different parts of the project in preparation for their team's competition. Classroom teachers, on the other hand, may struggle to fit robotics into the curriculum because they can have trouble seeing how robotics relates to their subject area, do not have lesson plans for integrating coding/robotics into their classes, and may not have the technical background to develop their own curriculum. Finally, in the school setting, school administration will set the priorities for a school, determine whether not there is time for robotics in the curriculum, and control the funds for materials; therefore administration needs to support robotics for educators to have the resources to purchase materials and feel empowered to teach it.

Overall, to address access, tools should be low-cost or operable on general-purpose hardware, require little physical space, and make efficient use of classroom time.

\subsubsection{Need for Engagement}
For those who can access robotics, a need for engagement becomes the next biggest focus. Both educators and students continuously mentioned that trial-and-error programming and development was a large source of frustration and a detractor from engagement. Specifically, fine-grained, imperative navigation code requires children check and recheck their robot against the same objective, and children get discouraged when they cannot make progress or bored when they repeat the same task with little success.

\begin{quote}
    “Oh, the most frustrating part of the project was probably—I'd have to test out the speed so many times. And then every time I had to—I had to plug it in and then it'd take 1 or 2 seconds to download it. Then I have to go to the finder and I'd always have to eject it, and then whenever it didn't work, I have to go back and change it again. And then I do that and then I got to keep on doing the same thing over and over until I get it right.” --Child 2
\end{quote}

Despite this frustration, robotics as an activity can inherently support engagement through active, project-based learning. We found that students enjoy the hands-on aspects of robotics, and the open-ended, goal-based problems that these activities support allow children to think critically and learn through the process of doing, rather than rote memorization or repetition. Educator 7 leverages this desire for hands-on activities to build excitement for learning and combat student fatigue.

\begin{quote}
    “There's a threshold there where kids kind of get burned out. And so what I've learned is to mix it up with the hands on. There has to be—when you're doing coding, there has to be a hands on a component.” --Educator 7
\end{quote}

Educators also deliberately support youths' engagement by providing choice in their learning. Within a robotics team, students often choose what aspects of the project they want to participate in (i.e., coding or building) and in the context of a broader technology classroom, several educators allow students to choose what kind of technology they engage with. These educators report that not all of their students will pick robotics, but those that do are more engaged because of that choice. Students, too, repeatedly expressed a desire for choice: they wanted kits of modular robots with a plethora of peripherals and the chance to design the courses and objectives that their robots take on. Child 5 described his ideal robotics kit as providing choice both in what you can build and how you can code.

\begin{quote}
    “I think it should be super customizable so it can be whatever they want. It can, like, use other resources from other kits if they have any. And they can program it in almost any language.” --Child 5
\end{quote}

Finally, the motivators for robotics can be a source of engagement as well. Many students reported feeling motivated by a feeling of success or accomplishment when they see the results of all of their hard work. Others said the the social aspects of robotics were motivating, and that connection to their peers and opportunities for collaboration made robotics more fun. 

\begin{quote}
    “I do FIRST Lego league...That was also really fun 'cause I did that with my friends.” --Child 1
\end{quote}

Competition, too, provides motivation for some students, who enjoy sharing their ideas with others or simply have a desire to win. However, not all participants appreciated competitive aspects of robotics because the competition objectives change the learning goals (e.g., time on presentation prep and annual theme-related social impact projects is time away from robotics), repetitive preparation (e.g., practicing a presentation) can be frustrating or boring, and the competitions themselves are in metropolitan areas, which can limit access for rural communities.

Overall, to support engagement, tools should provide students with choice, social interaction, and opportunities for hands-on activities.

\subsubsection{Impact of Autonomous Navigation}
In accordance with prior work, we used ``superpowers'' as a metaphor to encourage participants to think about AI \cite{holstein2017intelligent}. When participants were asked about a superpower that could make their robot navigate a course on its own with just one block/line of code (i.e., autonomously), they expressed split opinions. Some participants were enthusiastic about the idea because the superpower would make it easier for people to get started with robotics. That is, if educators do not need to know how to code in order to do robotics, they may be more inclined to use it in their classrooms. Similarly, autonomous navigation would expand the scope of potential projects; whereas robotics is currently limited to tracks or tables, autonomous robots could navigate the world and take on more complex or real-world problems. For instance, one student became excited about the possibility of creating a ``seeing eye robot'' for a person with visual impairments, which he would not be able to do with robot that had to be programmed to navigate each and every environment it might operate in.

On the other hand, current robotics teaches coding fundamentals, and some educators were concerned that integrating ML-based autonomous navigation could change these learning goals. Therefore, a robotics education approach leveraging autonomous navigation should make it easy for users of any background or expertise to get started, support a wide range of projects, and have clearly defined learning objectives which include opportunities to engage with coding fundamentals.
